Two Hands Are Better Than One: Resolving Hand to Hand Intersections via Occupancy Networks

3D hand pose estimation from images has seen considerable interest from the literature, with new methods improving overall 3D accuracy. One current challenge is to address hand-to-hand interaction where self-occlusions and finger articulation pose a significant problem to estimation. Little work has applied physical constraints that minimize the hand intersections that occur as a result of noisy estimation. This work addresses the intersection of hands by exploiting an occupancy network that represents the hand's volume as a continuous manifold. This allows us to model the probability distribution of points being inside a hand. We designed an intersection loss function to minimize the likelihood of hand-to-point intersections. Moreover, we propose a new hand mesh parameterization that is superior to the commonly used MANO model in many respects including lower mesh complexity, underlying 3D skeleton extraction, watertightness, etc. On the benchmark InterHand2.6M dataset, the models trained using our intersection loss achieve better results than the state-of-the-art by significantly decreasing the number of hand intersections while lowering the mean per-joint positional error. Additionally, we demonstrate superior performance for 3D hand uplift on Re:InterHand and SMILE datasets and show reduced hand-to-hand intersections for complex domains such as sign-language pose estimation.

==> reviewers.tex <==
AC: concerns about
1. the paper's organization, 
2. motivation/novelty statement, and 
3. reproducibility (due to a lack of methodological details or openly shared code).

Reviewer 1:
The main weakness is that the work is not detailed enough to be reproducible.

Reviewer 2:
- The introduction fails to clearly state which are the main contributions of this paper. The introduction mix together the description of previous works with a vague description of the aim of this work
- The description of the methodology is also confused. It fails to clearly state the limitation of current methods and evidence where this paper provides something new.
- The experimentation fails to evidence the limitations of the methods and the cases where it does not work properly or evidently fails.
- More details of the method should be reported to improve the reproducibility of the approach.
- substantially improve the paper organization clearly separating the previous work from the contribution of this paper. Novelty should be clearly stated

Reviewer 3:
- The presentation could be improved. The paper would also benefit from a better organization. Some points to consider:
o The focus of the presentation is clearly on the InterHand2.6M dataset and for some time when reading the paper I was under the impression that this is the only datasets used. Only in Section III-C I realized this was tested on more dataset. The authors may consider highlighting this fact more explicitly earlier in the paper and mention the datasets in the abstract already.
o The motivation in Section I-B that described the idea at a high level is somewhat modest and with incomplete information. I did not really understand how the approach works from this description. I would at least mention the 3D CNN predictor and mentioned explicitly what the output of the occupancy network is at this stage. Which component is predicting the hand mesh at the end?
o The 3D CNN predictor is never described. What is it? Are these the baseline models? The same applies to the occupancy networks. What is? Encoder-decoder model scan be anything, from different CNNs, UNets, transformers or more exotic model topologies.

- The limitation of the model are not discussed. No failure cases are presented that would provide the basis for discussions.
- What is the computation complexity of the proposed approach?
- The validation is somewhat modest. The related work section discussed multiple models fort his task, but only two are considered for the evaluation. I understand that these two are compatible with the claimed contribution allowing the authors to show how their solutions work, but how that compares to other solutions is not clear from the experiments.


Final:
= Specific:
- reproducibility (due to a lack of methodological details or openly shared code)
- motivation/aim statement
- novelty statement
				- previous/related work separation
				- limitations of the work
- computational complexity
- CNN model description



= Abstract:
- Organisation


==> tables/interhand.tex <==
% \begin{table}[ht]
% \centering
% \caption{Caption above}
% \begin{tabular}{crr}
% % \begin{tabular}{@{}cr@{}}
% \rowcolor{tablegray}\hline%\toprule
% Method & MPJPE & MRRPE \\\hline
% Moon~{\etal}~\cite{Moon_2020_ECCV_InterHand2.6M} & 16.02 & 32.57 \\
% Fan~{\etal}~\cite{fan2021digit} & 14.27 & \\
% Meng~{\etal}~\cite{meng2022hdr} & 13.12 & \\
% Jiang~{\etal}~\cite{jiang2023a2jtransformer} & 10.96 &  \\
% Li~{\etal}~\cite{Li2022intaghand} & 9.40 & \\
% Li~{\etal}~\cite{Li2022intaghand} & 14.38* & \\
% Yu~{\etal}~\cite{yu2023acr} & 8.41 & \\
% Proposed &  & \\
% \hline
% \end{tabular}
% \label{table:human36}
% \end{table}

\begin{table}[ht]
\centering
\caption{Comparison of~{\sota} models and their updated versions trained with intersection loss in terms of a number of intersections.
The second column indicates the amount of intersections found via the ray-casting algorithm (Ray-C.), and the last four columns show the quantity of intersections determined by the occupancy network with different settings,~{\ie} testing single or flipped hands and density of points: ``S'' -- sparse, and ``D'' -- dense.
The ``\%'' row reports a percentage decrease in the amount of intersections for the proposed models. The total number of tested hand pairs is around 157000.}
% \vspace{-0.15cm}
\begin{tabular}{lrrrrr}
\rowcolor{tablegray}\hline%\toprule
% Method & Ray-C. & S & Sym + S & D & Sym + D \\\hline
&  & \multicolumn{2}{c}{Two (flipped) hands} & \multicolumn{2}{c}{Single}  \\
\rowcolor{tablegray}%\toprule
\multirow{-2}{*}{Method} & \multirow{-2}{*}{Ray-C.} & \multicolumn{1}{c}{D} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{D} & \multicolumn{1}{c}{S} \\\hline
A2J~\cite{Xiong_a2j} & 568856 & 312975 & 64118 & 167372 & 33842 \\
A2J+Ours & {\bf 472166} & {\bf 282440} & {\bf 54162} & {\bf 138766}  & {\bf 25369}  \\
\% & 17.00 & 9.75  & 15.53 & 17.09 & 25.04 \\
\hline
IH~\cite{Li2022intaghand} & 845776 & 531556& 103275 & 262232 &50528   \\
IH+Ours & {\bf 675385} & {\bf 427725} & {\bf 82595} & {\bf 212060} & {\bf 39892}\\
\% & 20.15 & 19.53 & 20.02 & 19.13 & 21.05 \\
\hline
\end{tabular}
\label{table:interhand}
\end{table}


\begin{table}[ht]
\centering
\caption{Comparison of~{\sota} models with and without intersections loss, and the ground truth hands on~\textsc{InterHand2.6M} dataset in terms of number of intersections found via ray-casting. Additionally, we filtered the data (around 21000 hand pairs) to require both ground truth hands to have the highest reconstruction confidence. The ``\%'' row denotes a percentage decrease in the number of intersections for models with the intersection loss function.}
% \vspace{-0.15cm}
% \begin{tabular}{lrrr|rrr}
% \rowcolor{tablegray}\hline%\toprule
%  & A2J & A2J* & GT & IH & IH* & GT \\\hline
% Ray-C. & 143344 & 96721  &  36348 & 228799 & 148378 & 36373 \\
% \% & \multicolumn{2}{c}{32.53} & & \multicolumn{2}{c}{35.15}  & \\\hline

\begin{tabular}{lrr|rr|r}
\rowcolor{tablegray}\hline%\toprule
 & \multicolumn{1}{c}{A2J~\cite{Xiong_a2j}} & \multicolumn{1}{c}{A2J+Ours} & \multicolumn{1}{c}{IH~\cite{Li2022intaghand}} & \multicolumn{1}{c}{IH+Ours} & \multicolumn{1}{c}{GT} \\\hline
Ray-C. & 143344 & 96721 & 228799 & 148378 & 36361 \\
\% & \multicolumn{2}{c|}{32.53} & \multicolumn{2}{c|}{35.15}  & \\\hline
\end{tabular}
\label{table:interhand_filtered}
\end{table}



